MPInspector: A Systematic and Automatic Approach for Evaluating the Security of IoT Messaging Protocols

Facilitated by messaging protocols (MP), many home devices are connected to the Internet, bringing convenience and accessibility to customers. However, most deployed MPs on IoT platforms are fragmented and are not implemented carefully to support secure communication. To the best of our knowledge, there is no systematic solution to perform automatic security checks on MP implementations yet. To bridge the gap, we present MPInspector, the first automatic and systematic solution for vetting the security of MP implementations. MPInspector combines model learning with formal analysis and operates in three stages: (a) using parameter semantics extraction and interaction logic extraction to automatically infer the state machine of an MP implementation, (b) generating security properties based on meta properties and the state machine, and (c) applying automatic property based formal verification to identify property violations. We evaluate MPInspector on three popular MPs, including MQTT, CoAP and AMQP, implemented on nine leading IoT platforms. It identifies 252 property violations, leveraging which we further identify eleven types of attacks under two realistic attack scenarios. In addition, we demonstrate that MPInspector is lightweight (the average overhead of end-to-end analysis is ~4.5 hours) and effective with a precision of 100% in identifying property violations.

==> experiments.tex <==
\section{Experiments}
We perform our experiments on a laptop computer with a 2.6 GHz 2-core Intel i5 processor and 8GB RAM, using Oracle' Java Runtime version 1.8 (64 bit) in its default settings. We build \texttt{MPInspector} in approximately 5k lines of Java code, 2k lines of JavaScript code and 1k Python code. When it comes to evaluation, we build ten MP implementation experiments and generated 6k lines of Tamarin code about the formalized Tamarin model of ten MP implementations. \texttt{MPInspector} will be open-source for more MP implementations exploration.

%1331+26 = 1357 lines codes for semantic analysis for mqtt

%824 line python code for translation 

%2825 line java code for MQTT state fuzzing

%653 line js code for amqp adapter and mapper

%539 line java code for coap adapter and mapper


\textbf{Evaluation subjects.}
To estimate the effectiveness of \texttt{MPInspector}, we test ten MP implementations for three MP protocols( MQTT, CoAP, CoAP). We perform our analysis on the middlewares so that the analysis can cover more devices in the real world that use these middlewares. A previous survey \cite{whyshouldbuildown} shows IoT vendors just simply deploy the middlewares instead of customization. As a result, the analysis on the middleware will very likely to be consistent with on the devices. As Table~\ref{platforms} lists platforms (middlewares) we evaluate, which are the most popular IoT platforms \cite{competitivelandscape}. As an example, Tuya Smart hosts 100 million smart devices and covers over 220 countries \cite{tuya}.

% \yuan{First state that middlewares are very popular, and many manufactures will produce their products from middlewares. Remember that I asked you once to find references/reports that say small manufactures don't usually do customization on middleware. Then you can convince people that validating security attacks on middleware is a reasonable solution.} 
In our experiments, we register middlewares from the listed IoT platforms and accomplish the MP communication between the server and devices based on the middlewares. Then we apply our framework to perform analysis. 
% In addition, we validate our findings on the real world devices from Tuya Smart under their permissions.%and we validate our MQTT finding in Tuya Smart under their permission.

\begin{table}[!htbp]
\centering
 \caption{Tested MP implementations with their platforms }
 \label{platforms}
\scriptsize
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Platform} & \textbf{URL} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}MP\\ Version\end{tabular}}} \\ \hline
Google IoT Core & https://cloud.google.com/solutions/iot/ & MQTT V3.1.1\\ \hline
AWS IoT Core  & https://aws.amazon.com/iot/& MQTT V3.1.1\\ \hline
Azure IoT Hub  & https://azure.microsoft.com/services/iot-hub/ & MQTT V3.1.1\\ \hline
Bosch IoT Hub & https://developer.bosch-iot-suite.com& MQTT V3.1.1\\ \hline
Aliyun Cloud & https://iot.aliyun.com & MQTT V3.1.1  \\ \hline
Tuya Smart & https://en.tuya.com/cn/ & MQTT V3.1.1  \\ \hline
%Mosquitto & https://mosquitto.org/  & MQTTv5.0 \\ \hline
Mosquitto & https://mosquitto.org/ & MQTT V5.0\\ \hline
EMQ X & https://github.com/emqx/emqx-coap& CoAP  \\ \hline
Aliyun Cloud & https://iot.aliyun.com & CoAP \\ \hline
ActiveMQ &https://activemq.apache.org/ & AMQP V1.0  \\ \hline
\end{tabular}
\end{table}
\vspace{-2mm}

\textbf{Validation settings.} As for vulnerabilities and attack validation, we use the client SDK provided by the middleware to build potential victims. As for Tuya Smart who we have a partnership with, we validated our findings on the real device under their permission. We also build up scripts based on JavaScript to exploit the vulnerabilities and perform the attacks. Performed as the adversary, we manually checked those lemmas guided by the attack paths generated by the Tamarin prover using our scripts to see if we can acknowledge the secret or impersonated the agents in the communication between the servers with the client.

% message-oriented middleware

%We referred the MQTTv3.3.1 specification and MQTTv5.0 specification as well as the platform requirements to extract secerecy lemmas and authentication lemmas.

%\subsection{Experiment Settings}



% \yuan{Does the state fuzzing part overlap with the last section?}
% We use Learnlib 0.12.0 and Apache maven 3.6.3 for state fuzzing components and Graphviz 0.10.1 built in the module for visualization of state models. In semantic extracting component, we use SSLSplit 0.5.0 to collect the desired traffic and Java 1.8 for semantic extraction. 
% In the same time, we used python 3.7 to translate the state machine and desired properties into formal representations. Additionally, we used Tamarin 1.4.1 for automatically properties validation and python 3.7 for proving strategies designing.  %\yuan{Talk about open source. You can even post an anonymous link.}



==> findings_detail.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Findings}
\subsection{Attacks based on the property violations}\label{sec:findings}
%\wqy{this section is updated.}
%\todo{summery}
% \todo{every attack should be described as follows: introduction, the relation with the flaw, compare the IoT platforms and give out the reason, impact of the attack}

This section answers the question \textbf{RQ3}. Based on the property violations, we uncover eleven kinds of attacks on ten MP implementations and display the overview in Table~\ref{findings}. We find that MP implementations in our experiment are all vulnerable under two attack scenarios.  \wqy{Each platform is exposed to at least one attack. These attacks have serious consequences, such as sensitive data leak and malicious message injection. The detailed attacks are present as follows.}
\yuan{Need to give an overview of the attacks in the protocols/platforms. How bad is the situation overall?}
% We find that all protocol implementations can be exposed to MITM attacks under neighbor scenario while some MQTT protocol implementations additionally exposed to the replay attacks and AMQP protocol implementation is also exposed to synchronization attack. Under tenant scenarios, eight protocol implementations are exposed to client identity hijacking attacks. We also find protocol specific attacks on CoAP implementations that is reflection attack and the AMQP v1.0 protocol implementation with its special illegal occupation attack. There are also some attacks such as unauthorized topic subscription or unauthorized topic publish attacks we found on the three type protocols. 

%\includegraphics[scale=0.030]{pic/mark_all.png}
% \includegraphics[scale=0.030]{pic/mark_all.png}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
 \caption{ The overview of attacks based on violated properties (\protect\includegraphics[scale=0.030]{pic/mark_all.png}=validated, \protect\includegraphics[scale=0.030]{pic/mark_half.png}=partially validated)}
 \label{findings}
 \scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Scenario} & \textbf{Attacks} & \textbf{\begin{tabular}[c]{@{}c@{}}Affected\\ Protocol\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Affected\\ Platforms\end{tabular}} & \textbf{Related Pr.} & \textbf{\begin{tabular}[c]{@{}c@{}}Attack\\ Success\end{tabular}} \\ \hline
 & Man in the middle & All protocols & All platforms & MA1-MA9, AA1-AA13, CA1-CA8 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-6} 
 & Replay attack & \begin{tabular}[c]{@{}c@{}}MQTTv3.1.1\\ MQTTv5.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}Tuya Smart\\ Mosquitto\end{tabular} & MA1-MA9,MA10-MA11 (MQTT V5) & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-6} 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Neighbor\\ Scenario\end{tabular}} & Transfer sync. failure & AMQPv1.0 & ActiveMQ & AA1-AA9 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \hline
 &  & \begin{tabular}[c]{@{}c@{}}MQTTv3.1.1\\ MQTTv5.0\end{tabular} & \begin{tabular}[c]{@{}c@{}}Google IoT Core\\ AWS IoT Core\\ Aliyun Cloud\end{tabular} & MS1-MS7,MA1,MA3,MA5,MA7,MA9 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{3-6} 
 &  & AMQPv1.0 & ActiveMQ & AS1-AS5, AA1,AA3,AA5,AA7,AA9,AA11,AA13 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{3-6} 
 & \multirow{-5}{*}{Client Identity Hijacking} & CoAP & \begin{tabular}[c]{@{}c@{}}EMQ X\\ Aliyun Cloud\end{tabular} & CS1-CS11,CA1,CA3,CA5,CA7 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-6} 
 & Reflection attack & CoAP & \begin{tabular}[c]{@{}c@{}}EMQ X\\ Aliyun Cloud\end{tabular} & CS1,CA1,CA3,CA5,CA7 & \includegraphics[scale=0.030]{pic/mark_half.png} \\ \cline{2-6} 
 &  & MQTTv3.1.1 & AWS IoT Core & S5,MS7,MA3 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{3-6} 
 & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Malicious Topic\\ Subscription\end{tabular}} & AMQPv1.0 & ActiveMQ & AS2,AS4,AA9 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-6} 
 &  & MQTTv3.1.1 & AWS IoT Core & MS5,MS7-MS9,MA7 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{3-6} 
 & \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Malicious Topic\\ Publish\end{tabular}} & CoAP & EMQ X & CS1,CA3 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}Malicious Response\\ Topic Publish\end{tabular} & MQTTv5.0 & Mosquitto & MS5,MS7-9,MA7 &  \includegraphics[scale=0.030]{pic/mark_half.png} \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}Unauthorized Will\\ Message\end{tabular} & MQTTv3.1.1, MQTTv5.0 & \begin{tabular}[c]{@{}c@{}} AWS IoT Core\end{tabular} & MA1,MA10 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-6} 
 & \begin{tabular}[c]{@{}c@{}}Unauthorized Retained\\ Message\end{tabular} & MQTTv5.0 & Mosquitto & MA8, M11 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-6} 
\multirow{-19}{*}{\begin{tabular}[c]{@{}c@{}}Tenant\\ Scenario\end{tabular}} & Illegal occupation & AMQP1.0 & ActiveMQ & AS1,AA1,AA3 & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \hline
\end{tabular}
\end{table*}

% \subsubsection{Neighbor Scenario}
%\yuan{We should follow the same writing structure for each attack. 1) Violations->attacks: The reasons for these attacks, linking the property violations with the attacks. 2)Attacks Identified: What platforms are vulnerable, what are the consequences.  BTW, I think property violations are more specific than flaws. Maybe we should always refer to them as violations.3)validation of attacks. You can use textit to highlight the three parts.} \wqy{updated}

\textbf{Man in the middle.} Based on all the violated authentication properties in the neighbor scenario, a man-in-the-middle attack can be performed. The three MPs lack proper authentication mechanisms on both client side and server side.

\textit{Attacks identified:}  We find the ten MP implementations are exposed to this attack. In each phase of MP, the adversary can sniff sensitive data to infringe the victim's privacy, drop the messages for the DoS attack and inject malicious messages to control the clients.

\textit{Validation of attacks:} We successfully launch these attacks on all MP implementations. We build scripts to impersonate server and client and connect to the victim server and client.

% MPInspector identifies that all the authentication properties on both client side and server side are violated in neighbor scenarios which suggested that the adversary can perform man-in-the-middle-attack and connect to the client impersonating the server and connect to the server impersonating the client. This result shows that those ten MP implementations have no appropriate mechanism to identify the malicious packets in all phases from the adversary. As a consequence, the adversary can drop the packets to perform DoS attacks and can sniff the sensitive data as well as inject some falsified data. It is worth mentioning that the adversary can perform a DoS attack on MQTT implementations to continually send CONNECT packet to the server which will make the victim client offline as we found in the state machine of all MQTT implementations that when the server received duplicate connection request over a network connection the server will disconnect the client. In our manual experiments, we have successfully performed the man-in-the-middle attacks on ten MP implementations combining several attack methods such as DNS hijacking and ARP spoof.
%  Combining those strategies nd DNS hijacking or ARP spoof, we validated that ten MP implementations are all exposed to this attack.

\textbf{Replay attack.} This attack is related to the authentication properties of all phases in MQTT. The authentication properties fail aliveness goal on MQTT implementations which suggests the server will accept messages that the client has sent before. The adversary only needs to collect and replay them to the server.

\textit{Attacks identified.} We identified that Tuya Smart and Mosquitto are exposed to this attack. This attack can replay all the packets in MQTT implementation including connecting to the server and send commands or telemetry data.

\textit{Validation of attacks:} we successfully launch this attack on Tuya Smart and Mosquitto. We collect the traffic by sniffing in the local network and replay them to the server or the client. They accept them and response to us.

% According to the violated authentication flaws on all interaction phases on MQTT protocols, we identify there are three MQTT implementations that are exposed to replay attacks. These MP implementations are running over TCP protocols and there are no mechanism such as changing token adopted by the CoAP protocols. So the adversary can simply sniff the phases and reply them whenever they want. We validate that Tuya IoT Smart and Mosquitto are exposed to the replay attacks.
%  while other MP implementations has adopt some time related or order related parameters to avoid replay attack.

\textbf{AMQP sync. failure.} MPInspector extracts the state machine of AMQP implementation on ActiveMQ and found that the participants in AMQP protocol interact in a strict order and the sender and receiver strictly maintain the packet ID called Delivery ID when sending TRANSFER packets. Combined with the violated authentication properties on all AMQP phases, the adversary can continuously send the wrong order packets or forged the TRANSFER packets with synchronized Delivery ID using the victim's identity which can easily kick the victim offline. Figure~\ref{fig:amqpdenialofservice} shows the AMQP synchronization attacks exploiting the Delivery ID. The broker and the victim are maintaining two strict counter recording the next outgoing delivery id and the next incoming delivery id, and the broker will break the connection with the victim when the delivery id is not equal to the next incoming delivery ID.

\textit{Attacks identified:} We identified the attack on ActiveMQ. This attack can cause the victim out of service.

\textit{Validation of attacks:} We develop an attack script using Ettercap \cite{ettercap} and we successfully kick the victim offline. 
%%% shoudl add property secrecy on containerid 
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.35\textwidth]{pic/attacks/attack_amqpdos.JPG}
    \caption{AMQP sync. failure in tenant scenario}
    \label{fig:amqpdenialofservice}
\end{figure}

\subsubsection{Tenant Scenario}

\textbf{Client Identity Hijacking.} MPInspector detects that the secrecy properties on the client identity are all violated in the tenant scenario. Additionally, the server side authentication properties are violated which suggests that the adversary can impersonate the victim device using its identity to connect to the server.  We name this attack as client identity hijacking. 

In the tenant scenario, the ownership of the device can be changed. Still, we find that the identity will not be changed in some MP implementations which can be exploited to perform client identity hijacking attack. Especially, MPInspector detects that MQTT implementations will disconnect the existing client when the server received a second connect request with ClientId of the current client. The adversary can use the victim's identities to connect the server and kick the victim out of connection. Then, he can additionally apply the client identity hijacking to continuously send the CONNECT request packet, causing the victim devices never to go online. Last, the adversary can impersonate the device to send messages to the server.


\textit{Attacks identified:} We successfully launch the attack on MQTT implementations on Google IoT Core, AWS IoT Core, Aliyun Cloud, Tuya Smart, Mosquitto, EMQ X and ActiveMQ. They hard-codes the credentials of the client into device SDKs and can not dynamically revoke or grant new credential to the device. These credentials are not changed in the tenant scenario, which are still exposed to the client identity hijacking attack.

\textit{Validation of attack:} We successfully launch this attack using our script with the victim's credentials. We successfully connect to the server and kick out the victim.

% According to the reliability properties MR2 analysis, Google IoT Core, AWS IoT Core, Azure IoT Hub, Aliyun Cloud and Tuya Smart will disconnect the victim devices when received a new session with CONNECT packet forged by the adversary and exposed to the DoS attack if the adversary continually send the connect messages. The adversary can also inject opposite sensor data to the server such as "the door is locked" to spoof the client in user side. This attack is based on the secrecy flaws on the identity parameters from all the MP implementations.

\textbf{Reflection attack.} A reflection attack is specific to the CoAP protocol which is running over UDP protocols. Considered the violated secrecy properties on the CoAP Uri and the violated authentication properties on the different phases on the server side, the adversary can forge packets using the victim's IP address and URI to send to the server and the server will respond to the victim as the Figure~\ref{fig:coapreflection} shows.

\textit{Attacks identified:} We identify the attacks on CoAP implementations on Aliyun Cloud and EMQ X. This attack may cause serious consequences. To illustrate, the adversary can forge a fake state such as "the temperature is over 40 $^{\circ}$C" and send to the server, the server will send the control command such as "open the window" to the victim, which is a potential risk. Moreover, the adversary can forge a packet to get considerable resources which will send to be a response to the client and may cause the client denial of device.

\textit{Validation of attack:} The attack is partially validated. We use source address spoofing to forge the CoAP packet and the victim successfully receives the unexpected response packets. According to our experiments, the amplify reflection parameters are 2.25 in Aliyun Cloud and 0.68 in EMQ X. It is because we adopt the basic configuration of EMQ X and Aliyun Cloud, where the broker only returned the response code without the device data that the amplify reflection parameters in EMQ X and Aliyun Cloud are small. We believe the IoT vendors will return more than 100 bytes data including the device states, device commands and the amplify reflection parameters will be larger. Besides, the bandwidths of the device are small and even sending continuous packets of 100 bytes size to the device can cause DoS attacks according to the previous work \cite{doshi2018machine}. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.3\textwidth]{pic/attacks/attack_coapfmi.JPG}
    \caption{CoAP reflection attack in tenant scenario}
    \label{fig:coapreflection}
\end{figure}




% This attack is based on the authentication flaws and the secrecy flaw on CoAP uri which enable the adversary forge the amplify packet using the victim's uri and the packet accepted by the server.

\textbf{Malicious topic subscription.} Based on secrecy property violation on topic name and the authentication property violation on the SUBSCRIBE phase, the adversary subscribes to the victim's topic using his own identity. It is also because the MP implementations lack of access control of the client with the topics. Take AMQP as an example, we can learn from the Figure~\ref{fig:amqpsecretdataleak} that the adversary can use his own identity noted ContainerId to subscribe to the victim's topic noted as the target node. When victim devices send their secret data, the broker will transfer the secret data to the adversary or the victim.
\begin{figure}[htb]
    \centering
    \includegraphics[width=0.4\textwidth]{pic/attacks/attack_amqpsecretdataleak.JPG}
    \caption{AMQP arbitrary topic subscription in ActiveMQ in the Remote Attack Scenario}
    \label{fig:amqpsecretdataleak}
\end{figure}
\textit{Attacks identified:} We identify this attack on AWS IoT Core and ActiveMQ. This attack can steal the victim's privacy. For example, the adversary can acknowledge the sensitive health data from healthcare devices.

% In the meanwhile, AMQP implementations from ActiveMQ also exposed to these vulnerabilities.
\textit{Validation of attack:} We successfully launch this attack and receive sensitive messages from the victim.

\textbf{Malicious topic publish.} Similarly, we found that some MP implementations allow the client to publish messages to an unauthorized topic. Based on the violated secrecy property on the topic name and the violated authentication property on the PUBLISH phase or CON\_PUT phase, the adversary can exploit these violations to connect to the server using his own identity but publish evil command to the victim's topic. It is also because there is a gap between the identity and authorization on the topic.


\textit{Attacks identified:} We identify these attacks on AWS IoT Core and EMQ X. This attack allows the adversary to inject malicious messages such as sending "open the door" command.

\textit{Validation of attack:} We launch this attack on AWS IoT Core and EMQ X and successfully send malicious data to the victim.


\textbf{ Unauthorized response message. }
%mqttv5 request/response allow publish the message to a topic
This attack is baesd on the new request/response mechanism introduced by MQTTv5. This mechanism allows the client publish a message with a response topic and correlation data. The client who received this message publishes the correlation data to the response topic. However, The adversary can inject falsified message to unauthorized topics by publishing a message to the victim with a response topic. The victim is authorized to the response topic. Table~\ref{findings} shows the procedure of this attack which is based on the secrecy property violation on the victim's topic.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.3\textwidth]{pic/attacks/attack_mqtt5.JPG}
    \caption{MQTTv5 unauthorized response topic publish in tenant scenario}
    \label{fig:mqtt5attacks}
\end{figure}

\textit{Attacks identified:} This attack is identified on Mosquitto as it supports the MQTT V5.0.
%有点不会表述，mosquitto允许发送response topic但是他们的client还没有实现request的功能

\textit{Validation of attack:} This attack is partially validate as the client in Mosquitto partially accomplish the request/response mechanism. We use our script to simulate the victim and accomplish the request/response mechanism. We successfully launch the attack as the broker dose not check the authority of the response topic.

\textbf{Malicious will message and retained Message. } Based on the violated authentication properties on the CONNECT phase and PUBLISH phase, we identify the malicious will message and retain message attack. These two attacks are the same as the previous work in  \cite{mqttburglars}.

These two attacks are as follows: when the adversary has the temporary access control of the device, he registered will message by sending carefully constructed CONNECT packet and retained message by sending deliberately constructed PUBLISH packet in the server. The retained message will be sent when a victim registered the related topic and the will message will be sent when the adversary suddenly goes offline. Then he lost his control of the device and does not have the authority of the will message and retained message. However, victim devices can receive these two messages. 

\textit{Attacks identified:} We find AWS IoT Core are still exposed to the unauthorized will message attack and Mosquitto is still exposed to the unauthorized retained message attack.

\textit{Validation of attack:} We successful launch these two attacks on AWS IoT Core.

% as these two attacks have to performed in the interaction in which  two clients with a server are participated. We manually checked these two attacks and used our formalization module to make formal analysis which shows these two attacks are related to the secrecy flaws on the victim's topic, the authentication flaws on will message publish phase and retained message publish phase. It is worth mentioning that the retained message mechanism has been forbidden by most MP implementations except for the Mosquitto and the will message attack can be performed in AWS IoT Core. Furthermore, MQTT v5.0 has introduce the properties for most phases in MQTT protocol which can be utilized by the MP implementations to perform authorizations to avoid these unauthorized message publish attacks.

\textbf{Illegal occupation.} The adversary can exploit the violated secrecy property on the victim's ContainerId and the violated authentication property to perform illegal occupation attacks on AMQP. As Figure~\ref{fig:amqpio} shows, the server that received duplicate OPEN packet within the same ContainerId of the victim will close the connection but will not update the session state. When the client reconnects to the server, the server believes that the client with ContainerId of the victim has already connected and rejects the victim's connect request.

% on AMQP connection phases to make the victim never be able to connect the server.

% We also find the illegal occupation attack on the AMQP implementation from ActiveMQ. As Figure~\ref{fig:amqpio} shows, the implementation has flaw in the client identity management where the server that received duplicate OPEN packet within a client identity noted as ContainerId of victim will close the connection but will not update the session state and when the client reconnect to the server, the server will believe that the client with ContainerId of victim has already connected and reject the victim's connect request. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.35\textwidth]{pic/attacks/attack_amqpio.png}
    \caption{AMQP Illegal Occupation attack in tenant scenario}
    \label{fig:amqpio}
\end{figure}\textbf{}

\textit{Attacks identified:} We identify this attack on ActiveMQ and we believe this attack is severe. The adversary can use the ContainerId to register the client on their cloud and make the victim never connect to the broker unless the broker resets. 

\textit{Validation of attack:} We use our script to successfully launch this attack and the target victim can not connect to the broker anymore.

\iffalse
\discuss{I am not sure if this subsection is appropriate. I delete it.}
\subsection{Comparison between different platforms and protocols}
The attack result we identified in ten MP implementations are complicated and we have concluded that there are common attacks in all MP implementations and there are special attacks that is protocol specific due to their features.

\textbf{Common attacks.} We have found the SSL/TLS are the fundamental security mechanism which are recommended by the three MP specifications, however, some platforms still allow the unsafe connection on TCP protocols, resulted in the replay attacks. The CoAP implementations and AMQP implementations are safe from replay attacks as they have used packet id to identify the packets while MQTT implementations didn't adopted packet id in CONNECT and DISCONNECT phases. We also find the specification violation on the transmitted message in the three messaging protocol. The IoT platforms transfer the message in plain text which leak the clients' privacy.

Client identity hijacking has influenced all three types of messaging protocols as the credential are unchanged in tenant scenario in the IoT platform designs which should be dynamically granted and revoked.

Moreover, the three IoT protocols all suffered the topic related attacks, the topic should be bound with the identity of the client and the access control are not strictly deployed in some platforms in three messaging protocols by reason of lacking fine-grained access control strategies design.

\textbf{Protocol specific attacks.} As the AMQP protocols designed the most complicated connection procedure including 13 phases in the three protocols, these phases can be exploited by the adversary to cause the denial of attacks as their packets may not be carefully handled by the server. We also find that the AMQP protocol suffered the illegal occupation attacks as the adversary can exploit the OPEN phase and registered all the container id in the server and the victim can not connect to the server as the container id of victims are already occupied by the adversary. This is in virtue of the implementation flaws. The CoAP implementations have special attacks called reflection attack as the protocol are running over UDP protocols and the attack is common on UDP protocols. Moreover, MQTTv5.0 introduce a new request/response mechanism also may introduce the attack which the adversary can exploited the unauthorized response topic, owing to the missing inspection on the response topics.
\fi

\subsubsection{Comparison with Burglars' IoT Paradise}\label{sec:comparison}
% \yuan{Need to update the table to be consistent with our text. Also, add a note that [39] only analyzed one protocol manually.}
\begin{table}[htb]
\centering
 \caption{ Our results compared with \cite{mqttburglars} in MQTT ((\protect\includegraphics[scale=0.030]{pic/mark_all.png}=detected, \protect\includegraphics[scale=0.030]{pic/mark_null.png}=not detected)) }
 \textsubscript{}
 \label{tab:findingcomparison}
 \footnotesize
 \begin{tabular}{|c|c|c|c|}
\hline
\textbf{Scenario} & \textbf{Types of Attacks} & \textbf{\begin{tabular}[c]{@{}c@{}} \cite{mqttburglars}\end{tabular}} & \textbf{MPInspector} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Neighbor\\ Scenario\end{tabular}} & \textbf{Man in the Middle} & \includegraphics[scale=0.030]{pic/mark_null.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-4} 
 & \textbf{Replay Attack} & \includegraphics[scale=0.030]{pic/mark_null.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}Tenant\\ Scenario\end{tabular}} & \textbf{Unauthorized Will Message} & \includegraphics[scale=0.030]{pic/mark_all.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-4} 
 & \textbf{Malicious Retained Message} & \includegraphics[scale=0.030]{pic/mark_all.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-4} 
 & \textbf{Client Identity Hijacking} & \includegraphics[scale=0.030]{pic/mark_all.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-4} 
 & \textbf{ClientId identification} & \includegraphics[scale=0.030]{pic/mark_all.png} & \includegraphics[scale=0.030]{pic/mark_null.png} \\ \cline{2-4} 
 & \textbf{Malicious Topic Subscription} & \includegraphics[scale=0.030]{pic/mark_all.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-4} 
 & \textbf{Malicious Topic Publish} & \includegraphics[scale=0.030]{pic/mark_null.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \cline{2-4} 
 & \textbf{Wildcard-topic Subscription} & \includegraphics[scale=0.030]{pic/mark_all.png} & \includegraphics[scale=0.030]{pic/mark_null.png} \\ \cline{2-4} 
 & \textbf{\begin{tabular}[c]{@{}c@{}}Unauthorized Response\\ Topic Publish\end{tabular}} & \includegraphics[scale=0.030]{pic/mark_null.png} & \includegraphics[scale=0.030]{pic/mark_all.png} \\ \hline
 \end{tabular}
\end{table}

%  \includegraphics[scale=0.030]{pic/mark_all.png}
%  \includegraphics[scale=0.030]{pic/mark_null.png}
%   \includegraphics[scale=0.030]{pic/mark_half.png}

We compare our results with the previous work \cite{mqttburglars} by Jia \emph{et al.} Our framework is automatic while Jia \emph{et al.} only analyzed the MQTT manually. In addition, we explore two versions of MQTT and extend our framework to perform analysis on CoAP and AMQP while they only analyzed MQTT V3.1.1. 
As for MQTT V3.1.1, we find four attacks that Jia \emph{et al.} didn't cover. We consider the neighbor scenario and the tenant scenario while they only considered the latter. MPInspector dose not cover two attacks. ClientId identification was taken to guess the victim's ClientId which is not MQTT implementation flaws and wildcard-topic subscription was validated by check the format of the topic which is related to the understanding of the bit-wise parameters. MPInspector are designed for interaction logic analysis and the bit-wise parameters or words are not checked.


% We consider two realistic scenarios including neighbor scenario and tenant scenario while Jia \emph{et al.} in \cite{mqttburglars} only considered the tenant threat model. We find two types of attacks in the neighbor scenario and the man-in-the-middle attacks affected all MQTT implementations. In tenant scenario, Jia \emph{et al.} and we have four overlapped findings including client identity hijacking, unauthorized topic publish, unauthorized will message and unauthorized retained message. 

% It is worth mentioning that we explored two version including the latest 5.0 version of MQTT and extend our framework to perform analysis on CoAP and AMQP. We find more attacks than the the previous work \cite{mqttburglars}. Further, our framework is automatic while Jia \emph{et al.} only analyzed the MQTT manually. MPInspector can also identify the flaws which lead to the attacks, which can help developers fix their problem easily.
%\yuan{They only consider the tenant threat model, while we also consider neighbor threat model, we should point it out in the table, and also emphasize in the text.} 

% \textbf{Connection Relay. }

% Combined with DoS attack and server spoof, one of our exposed attacks called connection relay is stitched with a relay attack with which an adversary impersonates the victim server to connect the device. All the MQTT implementations are affected by the attack.


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{pic/attacks/attack_connectionrelay.JPG}
%     \caption{MQTT denial of service attack in tenant scenario}
%     \label{fig:connectionrelay}
% \end{figure}

% As the Figure~\ref{fig:connectionrelay} shows, the adversary first performs the denial of service attack by sending CONNECT packet in MQTT implementations or packets with asynchronous in AMQP implementations to server. The victim client will be offline and the adversary are able to connect with the broker impersonating the victim. Then, the adversary applied ARP spoof or DNS hijacking to connect with the victim impersonating the server. At last, all the messages sent by device will delivered to server by the adversary and all the messages sent by server will delivered to client by the adversary.







% % \yuan{This section is very long. We can have findings as a separate section instead of subsection.}
% We now present our findings on the attack vector in two attack scenarios based on the violated lemmas addressed in the former.

% \yuan{When you answer the research questions, you should follow the same order as you asked the questions, and point out which question you want to answer. In addition, when you have many different kinds of attacks, it is always good to summarize the findings first, before diving into the details. For example, please give an overview of the performance of the tool, and then talk about the details.}

% \yuan{We'd better have a case study if we can.}

% \textbf{Denial of Service.} %用重放实现disconnect，
% %%场景2下发起connect连接
% %发起disconnect+
% In this attack, the adversary can leverage some properties to force the victim offline with the brokers. 
% % According to our results of reliability properties analysis, all IoT platforms obey the MQTT specification that the server will disconnect the device when receives duplication CONNECT packets. In local network scenario, the adversary can perform connection relay attacks and forge fake CONNECT packet to the server, which will make the device out of service.

% % Additionally, the adversary can also perform the DoS attack by intercepting all the SUBSCRIBE, PUBLISH packets. However, the user can reboot the device and increase the adversary' cost because the adversary have to perform the MITM attack again.
% In remote network scenario, the adversary can send CONNECT packet with the parameters he collected previously to the server. The parameters will never change even when the devices are rebooted and the parameters are validated to fail the secrecy property in remote network scenario. According to the reliability properties analysis, Google IoT Core, AWS IoT Core, Azure IoT Hub, Aliyun Cloud and Tuya Smart will disconnect the victim devices when received a new session with CONNECT packet forged by the adversary. So, it is realistic to perform denial of service in remote network scenario by building new session with CONNECT packet to the server continuously.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.35\textwidth]{pic/attacks/attack_amqpdos.JPG}
%     \caption{AMQP denial of service attack in tenant scenario}
%     \label{fig:amqpdenialofservice}
% \end{figure}
% In AMQP implementations, the adversary can send forged message with a asynchronous delivery id to the broker using the victim's identity. As Figure~\ref{fig:amqpdenialofservice} shows, the broker and the victim are maintaining two strict counter recording the next outgoing delivery id and the next incoming delivery id, and the broker will break the connection with the victim when the delivery id is not equal to the next incoming delivery id. So, the denial of service can be performed by the adversary can send forged message with a asynchronous delivery id to the broker.

% \textbf{Connection Relay} One of our exposed attacks is stitched with a relay attack with which an adversary impersonates the victim server to connect the device. All the MP implementations are affected by the attack.

% In all three MP implementations, there are some implementations running over TCP protocols, which are easily to be exploited by the adversary in local scenarios, such as Aliyun Cloud, Tuya Smart, Poho MQTT Broker, Node-CoAP and ActiveMQ. The adversary can perform DNS hijacking or ARP spoof to spoof the device to connect with the adversary instead of the server.

% Although some implementations have adopted TLS protocol including Google IoT Core, AWS IoT Core, Azure IoT Hub, Bosch IoT Hub and Aliyun Cloud, they lack proper configurations on TLS protocols. In the MQTT implementations of Google IoT Core, Azure IoT Hub, Bosch IoT Hub and Aliyun Cloud, the servers do not validate the client's certification, which indicated that the adversary only need extra effort to make the client trust the adversary's certification, such as non-checking of server' certification in some clients, making device trust the the adversary's CA and applying a certificated which is signed by CA from the IoT platforms (supported by Bosch IoT Hub). Based on this attack, the adversary knows the session key and can decrypt the message that is sent by devices, and can modify the message before deliver to the server. All of the IoT platforms is under the risk of man in the middle attack. The attack works well in the simulate lab environment and we successfully validated the attack on a device we got from Tuya Smart using the research on Tuya Smart from \cite{tuyaattack} to establish the adversary's CA into the device.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{pic/attacks/attack_connectionrelay.JPG}
%     \caption{MQTT denial of service attack in tenant scenario}
%     \label{fig:connectionrelay}
% \end{figure}
% As the Figure~\ref{fig:connectionrelay} shows, the adversary first performs the denial of service attack by sending CONNECT packet in MQTT implementations or packets with asynchronous in AMQP implementations to server. The victim client will be offline and the adversary are able to connect with the broker impersonating the victim. Then, the adversary applied ARP spoof or DNS hijacking to connect with the victim impersonating the server. At last, all the messages sent by device will delivered to server by the adversary.

 





% \textbf{Secret Data Leak.}
% IoT platforms are using MPs to transfer sensor data and commands which should be confidential, as those data can leak the user's privacy, such as the health data and personal habits. However, in all platforms we found those data can be touched by the adversary.

% In MQTT implementations, the payload in PUBLISH packet is not encrypted which can be easily acknowledged by the adversary according the results of secrecy properties analysis in terms of local network scenarios. The PUBLISH packets are transferred on TLS protocol but they are visible to the server or the adversary who can perform man in the middle attacks, which also should be prohibited. All the MQTT IoT platform transfer the plain PUBLISH payload to the server except Tuya Smart. Tuya smart use a secret key to encrypt the payload of PUBLISH packets. However, in our experiment, Tuya Smart transfer the local key encrypted in the initial procedure which can be eavesdropped by the adversary in local network scenario. Similarly, the packets in the AMQP implementations in ActiveMQ and in the CoAP implementations in Node-CoAP broker transfer plain payload and are under the risk of secret data leak as they all failed the related security properties. In Aliyun Cloud, payload in CoAP protocols is encrypted by device secret and a temporarily generated random, which well protect the transported data.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{pic/attacks/attack_amqpsecretdataleak.JPG}
%     \caption{AMQP Secret Data Leak in ActiveMQ in the Remote Attack Scenario}
%     \label{fig:amqpsecretdataleak}
% \end{figure}

% It is worth mentioning that the adversary can also acknowledge the user secret in ActiveMQ in the remote attack scenario.
% As Figure~\ref{fig:amqpsecretdataleak} shows, the adversary can use his own identity noted ContainerId but the victim's topic noted as Targetname. when victim devices send its secret data, the broker will transfer the secret data to the adversary or the victim as the broker will not send the secret to any agent who connect with the victim's topic.





% \textbf{Replay Attack.}
% Replay attack is also common in our findings. When in the local scenarios, the adversary can collect all kinds of MP packets and replay them to achieve his purpose.

% In MQTT implementations, replay attack is easily to be performed by the adversary on Aliyun Cloud, Tuya Smart and Eclipse Paho broker which support MQTT running over TCP protocols as they failed the aliveness goal of authentication properties. All packets can be replayed by the adversary on Aliyun Cloud. The adversary can replay the CONNECT packet to connect with the server using victim's credential and can replay the PUBLISH packet to control the victim's device. On Tuya Smart, the PUBLISH packet contains a timestamp which cannot be replayed while other packets can be replayed in our attack experiment on a real device. While in CoAP and AMQP implementations, all types of packets in Node-CoAP and  can be replayed easily as well as publish related packets in Aliyun Cloud. In the meanwhile, Aliyun Cloud has adopted some security mechanisms such as timestamp in authentication packet, but turned out that the timestamp is not checked in the server side in our experiments, which indicated that the authentication packet can be replayed in Aliyun Cloud, too.


% % \begin{figure}[htbp]
% %     \centering
% %     \includegraphics[width=0.35\textwidth]{pic/attacks/attack_mqttreplayattack.JPG}
% %     \caption{MQTT Replay Attack}
% %     \label{fig:age}
% % \end{figure}


% %new attack
% \textbf{Falsified Messages Injecting. } In this attack, the adversary exploits the MP implementations and inject falsified message in the communication between the victim client and the server. It is obviously that all MP implementations are compromised to the attack when the adversary performs connection relay attack and following we showed the falsified message injection attack in remote network scenario.

% In MQTT implementations, We can learn from the results of authentication properties analysis that the SUBSCIRBE, UNSUBSCRIBE and PUBLISH packets fail the aliveness goal because they can be sent without authentication and they are authorized on the topic by their identities including the packetId in AWS IoT core and deviceName in Azure IoT Hub. The adversary who doesn't know the password or other secret credentials of client can bypass the CONNECT phase by using own client's credentials but send the SUBSCIRBE, UNSUBSCRIBE, PUBLISH, SUBSCRIBE DISCONNECT packets with false messages and victim' identities such as deviceId or packetId to the server. It can counterfeit device status to the server and can get the messages from the server side. AWS IoT platform, Azure IoT Hub, and Paho MQTT broker are affected in the remote network scenario. It is noted that our attack is different with \cite{mqttburglars} which find the authorization flaw on the platform identities and MQTT identities.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.35\textwidth]{pic/attacks/attack_mqttfmi.JPG}
%     \caption{MQTT falsified message injection in remote network}
%     \label{fig:age}
% \end{figure}

% %mqttv5 request/response allow publish message to a topic
% Moreover, MQTTv5 introduces a new request/response mechanism which may cause falsified message injection. This mechanism allows the client publish a message with response topic and correlation data and the client who received this message will publish the correaltion data to the response topic. However, this mechanism can be exploited by the adversary to inject falsified message to unauthorized topics by publishing a message to the victim with response topic that the victim is authorized such as the victim's topic as MQTTv5 allows the client send publish message to itself. The request/response mechanism makes the authorization more complicated.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\textwidth]{pic/attacks/attack_mqtt5.JPG}
%     \caption{MQTTv5 falsified message injection in tenant scenario}
%     \label{fig:amqpdenialofservice}
% \end{figure}
% When it reflect to CoAP and AMQP implementation, Node-CoAP and ActiveMQ violated all authentication properties, which indicates that the adversary can inject falsified messages to the broker by sending CoAP or AMQP packets with victim's identities in remote or local network. The falsified messages can be fake states or requests which can trigger the adversary desired response to the victims.



% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.35\textwidth]{pic/attacks/attack_coapfmi.JPG}
%     \caption{CoAP falsified message injection in tenant scenario}
%     \label{fig:amqpdenialofservice}
% \end{figure}

% However, CoAP implementation in Aliyun Cloud adopts device secret and a temporary random to encrypted the message sent to the server, which protects the clients from the falsified message injection in local network. When considering the remote network and the adversary knowing the secret device, the adversary can use victims' identity and credentials to connect with the broker and send falsified message to the broker.

% % 
